StraIT: Non-autoregressive Generation with Stratified Image Transformer

We propose Stratified Image Transformer(StraIT), a pure non-autoregressive(NAR) generative model that demonstrates superiority in high-quality image synthesis over existing autoregressive(AR) and diffusion models(DMs). In contrast to the under-exploitation of visual characteristics in existing vision tokenizer, we leverage the hierarchical nature of images to encode visual tokens into stratified levels with emergent properties. Through the proposed image stratification that obtains an interlinked token pair, we alleviate the modeling difficulty and lift the generative power of NAR models. Our experiments demonstrate that StraIT significantly improves NAR generation and out-performs existing DMs and AR methods while being order-of-magnitude faster, achieving FID scores of 3.96 at 256*256 resolution on ImageNet without leveraging any guidance in sampling or auxiliary image classifiers. When equipped with classifier-free guidance, our method achieves an FID of 3.36 and IS of 259.3. In addition, we illustrate the decoupled modeling process of StraIT generation, showing its compelling properties on applications including domain transfer.

==> sections/abstract.tex <==
\begin{abstract}

    We propose Stratified Image Transformer~(StraIT), a pure non-autoregressive~(NAR) generative model that firstly demonstrates superiority in high quality image synthesis over existing autoregressive~(AR) and diffusion models~(DMs). In this work, we dissect reasons that previously hinder the development of NAR models, in particular, the under-exploitation of visual characteristics in tokenization, and the increased complexity of handling longer sequences in a non-autoregressive manner. Through image stratification that obtains a masterful token pair, we alleviate the modeling difficulty and push forward the generative power of NAR models. Our experiments demonstrate that StraIT significantly improves NAR generation and firstly out-performs existing DMs and AR methods on the challenging ImageNet dataset, achieving FID scores of 3.96 at 256$\times$256 resolution without leveraging any guidance in sampling or auxiliary image classifiers. When equipped with classifier free guidance strategy to reduce compounding decoding error, our method achieves a FID of 3.36 and IS of 259.3. Besides, we illustrate the decoupled modeling process of StraIT generation, showing its compelling properties on domain transfer. 
\end{abstract}

